General Recursion and Formal Topology

It is well known that general recursion cannot be expressed within Martin-Loef's type theory and various approaches have been proposed to overcome this problem still maintaining the termination of the computation of the typable terms. In this work we propose a new approach to this problem based on the use of inductively generated formal topologies.

==> eptcsdata.tex <==
\providecommand{\firstpage}{65}
\providecommand{\publicationstatus}{A. Bove, E. Komendantskaya and M. Niqui (Eds.)\\
Partiality and Recursion in Interactive Theorem Provers.
\\
EPTCS 43, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.43.5}{10.4204/EPTCS.43.5}}

